Hacky Racers: Exploiting Instruction-Level Parallelism to Generate Stealthy Fine-Grained Timers

Side-channel attacks pose serious threats to many security models, especially sandbox-based browsers. While transient-execution side channels in out-of-order processors have previously been blamed for vulnerabilities such as Spectre and Meltdown, we show that in fact, the capability of out-of-order execution \emph{itself} to cause mayhem is far more general. We develop Hacky Racers, a new type of timing gadget that uses instruction-level parallelism, another key feature of out-of-order execution, to measure arbitrary fine-grained timing differences, even in the presence of highly restricted JavaScript sandbox environments. While such environments try to mitigate timing side channels by reducing timer precision and removing language features such as \textit{SharedArrayBuffer} that can be used to indirectly generate timers via thread-level parallelism, no such restrictions can be designed to limit Hacky Racers. We also design versions of Hacky Racers that require no misspeculation whatsoever, demonstrating that transient execution is not the only threat to security from modern microarchitectural performance optimization. We use Hacky Racers to construct novel \textit{backwards-in-time} Spectre gadgets, which break many hardware countermeasures in the literature by leaking secrets before misspeculation is discovered. We also use them to generate the first known last-level cache eviction set generator in JavaScript that does not require \textit{SharedArrayBuffer} support.

==> sections/artefact.tex <==
\appendix
\newpage
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

Our artifact provides source code and scripts for four timing side-channel experiments mentioned in this paper, corresponding to sections \ref{sec: JS backward-in-time} to \ref{sec:othermags}, and each demonstrates the efficiency and portability of either/both Racing and Magnifier Gadgets. Our results should be evaluated on an Intel or AMD x86 machine (we used an i7-8750h, but systems of a similar architecture will work out-of-the-box). Migration to systems with other ISAs or significantly different micro-architectures require minor source-code modifications.

\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}
  \item {\bf Algorithm: } ILP-based magnifiers, SpectreBack attack \& Hacky Racer-integrated Prime+Scope~\cite{primescope}.
  \item {\bf Program: } Arbitrary Replacement Magnifier Gadget (sec \ref{sec: Arbitrary Replacement Gadget}), Arithmetic-Operation-Only Magnifier Gadget (sec \ref{sec: Arbitrary Replacement Gadget}), SpectreBack Attack \& Prime+Scope-based LLC Eviction Set profiling.
  \item {\bf Compilation: } Succeeded on all tested compilers (gcc-6,7,8,10 \& clang 10).
  \item {\bf Binary: } Can be generated from script and source code.
  \item {\bf Run-time environment:} Linux shell scripts.
  \item {\bf Hardware: } ILP-based magnifiers succeeded on tested Intel (Skylake, Haswell, Coffee Lake) and AMD (Zen 2, Zen3) CPUs. SpectreBack attack \& Hacky Racer-integrated EV set profiling are successfully tested on an i7-8750h CPU. Other CPUs should give similar results.
  \item {\bf Run-time environment: } Provided scripts are for Linux, but the source code and script could be applied to others with minor modifications. The SpectreBack attack requires Chrome 88 (can be altered to other browsers by changing parameters), Python, and flask package.
  \item {\bf Output: } Accumulated timing difference versus magnify rounds for those two magnifier gadgets. The data points should be similar to that in figure \ref{fig: sets reuse results} and \ref{fig: arithmetic magnifier result}. A screenshot of the expected output of SpectreBack attack is stored in the Github repo. The output of Hacky Racer-integrated Prime+Scope should have the same output to the original Prime+Scope, showing whether an LLC EV is successfully generated or not.
  \item {\bf Publicly available?: } Yes, at \url{https://zenodo.org/badge/latestdoi/551660156}.
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}
Our source code and scripts are available on Github: \url{https://github.com/FxPiGaAo/Hacky-Racer}

\subsubsection{Hardware dependencies}
We recommend to run our testing on an Intel Coffee Lake (an i7-8750H was our main test system, but other recent Intel systems should deliver similar results) or AMD ZEN 2/3 (we used Ryzen 5900hx). For the Hacky Racer-integrated EV-set profiling attack, our prototype requires an inclusive LLC (as featured on most recent Intel cores, but not on Ryzen cores), so AMD systems can only be used to replicate the other three attacks out-of-the-box.

\subsubsection{Software dependencies}
Our source code assumes Ubuntu 18.04 on x86-64 systems. Other Linux-based operating systems should also work. To run the SpectreBack attack experiment, python, flask and Chrome 88 are required to be installed (instructions given in the repository).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

You can clone our source code and scripts from Github:
\textit{git clone https://github.com/FxPiGaAo/Hacky-Racer.git}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}
Before running any experiments, we recommend to fix the CPU frequency following the instruction given in the \textit{README.md} to eliminate the affect from DVFS. Any value is suitable (and the attacks will succeed without doing this, but with more noise), but we ran at 2GHz. For both the Arbitrary Replacement Magnifier Gadget and SpectreBack attack, multiple attempts may be required for success, as background processes might interfere with the cache and affect the result.

To run the Arithmetic-Operation-Only Magnifier Gadget, enter the \textit{Arithmetic-Operation-Only Magnifier Gadget} directory and execute \textit{./test.sh}. This test should take around 1min.

To run the Arbitrary Replacement Magnifier Gadget, enter the \textit{Arbitrary Replacement Magnifier Gadget} directory, and execute \textit{make; ./arbitrary}. This test should take around 30s.

To run the SpectreBack attack, please follow the instruction provided in \textit{spectre.js/README.md} step-by-step to install the pre-requirements (chrome 88 \& flask) and execute the attack. This test should take around 20 minutes to set up the requirements and another 5 minutes to go through the attack.

To run the Prime+Scope integrated with Hacky Racers, please follow the instructions given in \textit{PRIME-SCOPE-hackyracer/README.md}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

The expected result of each experiments are put into the \textit{README.md} of each experiment's folder.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment Customization}
For the SpectreBack attack, minor code modifications can be applied to run it on different versions of Chrome or other browsers (as with the \url{https://leaky.page/} code is it based on). Specifically, only offset parameters at lines 103 - 105 are specific to Chrome 88.

For the Arbitrary Replacement Magnifier Gadget, parameters such as cache offset, prefetch distance, and number of cache accesses within each set per round, can be easily modified in the source code.

For the Arithmetic-Operation-Only Magnifier Gadget, path lengths can be modified in either the \textit{magnify()} in \textit{arithmetic\_source.c} or the \textit{test.sh}. The operation type in the racing stage can also be changed by modifying the assembly code part in \textit{magnify()}.

For the Prime+Scope integrated with Hacky Racers, a magnifier gadget can be implemented after the racing gadget through source code modification if necessary.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Methodology}
The artifact for this paper was reviewed according to the guidelines at \url{https://sites.google.com/stanford.edu/asplos23aec/home}.
